The PTI Carbon Star Angular Size Survey: Effective Temperatures and Non-Sphericity

We report new interferometric angular diameter observations of 41 carbon stars observed with the Palomar Testbed Interferometer (PTI). Two of these stars are CH carbon stars and represent the first such measurements for this subtype. Of these, 39 have Yamashita (1972,1975) spectral classes and are of sufficiently high quality that we may determine the dependence of effective temperature on spectral type. We find that there is a tendency for the effective temperature to increase with increasing temperature index by ~120K per step, starting at T_EFF ~= 2500K for C3,y, although there is a large amount of scatter about this relationship. Overall, the median effective temperature for the carbon star sample is found to be 2800 +- 270K, and the median linear radius is 360 +- 100 R_SUN. We also find agreement on average within 15K with the T_EFF determinations of Bergeat (2001,2002a,b), and a refinement of carbon star angular size prediction based on V & K magnitudes is presented that is good to an rms of 12%. A subsample of our stars have sufficient {u,v} coverage to permit non-spherical modeling of their photospheres, and a general tendency for detection of statistically significant departures from sphericity with increasing signal-to-noise of the interferometric data is seen. The implications of most - and potentially all - carbon stars being non-spherical is considered in the context of surface inhomogeneities and a rotation-mass loss connection.

==> table_target_variability.tex <==
%% LaTeX deluxetable generator for the AASTeX package.
%% Written by Greg Schwarz (5/1/2001).

%% Table generated: Mon Sep  6 22:47:06 2010

%% Remove the two lines and the last line if you want
%% want to incorporate this table into another LaTex document.
%\documentclass[twocolumn]{emulateapj}
%\begin{document}

%% The values (usually only l,r and c) in the last part of
%% \begin{deluxetable}{} command tell LaTeX how many columns
%% there are and how to align them.
%\begin{deluxetable*}{llcccc}
\begin{deluxetable}{llcccc}
\tabletypesize{\scriptsize}											

%% Keep a portrait orientation

%% Over-ride the default font size
%% Use Default (12pt)

%% Use \tablewidth{?pt} to over-ride the default table width.
%% If you are unhappy with the default look at the end of the
%% *.log file to see what the default was set at before adjusting
%% this value.

%% This is the title of the table.
\tablecaption{Target variability as characterized by the GCVS, the AFOEV database, and {\it Hipparcos}.\label{tab_target_variability}}

%% This command over-rides LaTeX's natural table count
%% and replaces it with this number.  LaTeX will increment
%% all other tables after this table based on this number


%% The \tablehead gives provides the column headers.  It
%% is currently set up so that the column labels are on the
%% top line and the units surrounded by ()s are in the
%% bottom line.  You may add more header information by writing
%% another line between these lines. For each column that requries
%% extra information be sure to include a \colhead{text} command
%% and remember to end any extra lines with \\ and include the
%% correct number of &s.
\tablehead{
\colhead{} & \multicolumn{3}{c}{GCVS\tablenotemark{a}}  & \colhead{AFOEV} & \colhead{HIP} \\
\colhead{Star} & \colhead{Var} & \colhead{Amp} & \colhead{Band} & \colhead{Amp} & \colhead{Amp} \\
\colhead{ID} & \colhead{Type} & \colhead{[mag]} & \colhead{} & \colhead{[mag]} & \colhead{[mag]} \\
}
%% All data must appear between the \startdata and \enddata commands
\startdata
HD225217 & LC & 0.50 & V & 0.80 & 0.23 \\
HD2342 & SR & 1.90 & p & 1.80 & 0.36 \\
HD19881 & SRB: & 0.60 & V & 1.10 & 0.28 \\
IRC+40067 & LB: & 0.60 & p &  &  \\
HD280188 & SRA: & 1.01 & B & 1.10 & 0.26 \\
HD33016 & LB & 0.70 & V & 0.90 & 0.28 \\
HD34467 & LB & 1.05 & B & 0.60 & 0.15 \\
HIP25004 & SRA & 0.35 & Hp &  & 0.35 \\
HD38218 & SRB & 3.30 & V & 2.20 & 0.46 \\
HD247224 & LB & 1.90 & p & 1.40 &  \\
HD38572 & LB & 1.20 & B & 1.00 & 0.23 \\
HD38521 & SR: & 3.20 & p & 1.70 &  \\
HIP29896 & SR & 1.50 & V &  & 0.31 \\
HD45087 & LB & 2.20 & p &  &  \\
HIP31349 & LB & 1.20 & B & 1.00 & 0.54 \\
HD46321 & SRB & 1.30 & p & 1.50 & 0.16 \\
HD47883 & LB & 0.38 & V & 1.30 & 0.23 \\
HD48664 & LB & 2.00 & p &  &  \\
HD51620 & SRB & 2.19 & B & 2.40 & 0.39 \\
HD54361 & LB & 1.55 & V & 2.00 & 0.45 \\
HD57160 & SRB & 0.60 & p &  & 0.29 \\
HD59643 & SR+ZAND & 0.59 & V & 1.50 & 0.18 \\
HD60826 & LB & 0.50 & p & 0.55 &  \\
HD70072 & SRB & 2.80 & p & 2.75 &  \\
HD144578 & SRB & 4.70 & B & 2.60 & 1.61 \\
HD173291 & LB & 1.80 & V & 1.60 & 0.32 \\
HIP92194 & LB & 2.99 & B & 0.40 & 0.27 \\
HIP95777 & SRB & 3.50 & p & 2.50 & 0.29 \\
HD186047 & SRB & 1.70 & B & 1.70 & 0.26 \\
HIP99336 & LB & 2.20 & B & 0.80 & 0.32 \\
HD191783 & LB & 1.80 & V & 2.00 &  \\
HIP102764 & SR & 2.60 & B &  & 0.33 \\
HIP105539 & SRA & 1.10 & p & 0.80 & 0.51 \\
IRC+50399 & LB: & 1.10 & B &  &  \\
HD208512 & LB & 2.20 & B & 1.50 & 0.26 \\
HD208526 & SRB & 1.90 & p & 1.90 &  \\
HIP113715 & SRB & 2.20 & V & 1.40 & 0.64 \\
HD220870 & LB: & 1.00 & p & 1.30 & 0.26 \\
\enddata
%\tablenotetext{a}{Error bar is the formal fitting error.  For ensuing computations that make use of $\theta_{\rm UD}$, an error floor of $\pm 4.6\%$ will be used, as per the discussion at the end of \S \ref{sec_PA}.}
%\tablenotetext{b}{From the group designations in \citet{Bergeat2001A_A...369..178B}, as discussed in \S \ref{sec_BergeatCompare}.}
\tablenotetext{a}{Variability type and amplitude from the AAVSO Variability Index \citep{Watson2012yCat....102027W}; amplitude indicated as $V$-band, $B$-band, photographic (pg), or Hipparcos (Hp).}
%% Include any \tablenotetext{key}{text}, \tablerefs{ref list},
%% or \tablecomments{text} between the \enddata and
%% \end{deluxetable} commands

\tablecomments{No data available for HD30443, IRC+10158, HIP 95024.
AFOEV data has been selected for the available V-band data.
}

%% No \tablerefs indicated

\end{deluxetable}
%\end{deluxetable*}
%\end{document}


==> table_yamashita.tex <==
%% LaTeX deluxetable generator for the AASTeX package.
%% Written by Greg Schwarz (5/1/2001).

%% Table generated: Mon Sep  6 22:47:06 2010

%% Remove the two lines and the last line if you want
%% want to incorporate this table into another LaTex document.
%\documentclass[twocolumn]{emulateapj}
%\begin{document}

%% The values (usually only l,r and c) in the last part of
%% \begin{deluxetable}{} command tell LaTeX how many columns
%% there are and how to align them.
%\begin{deluxetable*}{llccc}
\begin{deluxetable}{llccc}
\tabletypesize{\scriptsize}											

%% Keep a portrait orientation

%% Over-ride the default font size
%% Use Default (12pt)

%% Use \tablewidth{?pt} to over-ride the default table width.
%% If you are unhappy with the default look at the end of the
%% *.log file to see what the default was set at before adjusting
%% this value.

%% This is the title of the table.
\tablecaption{Yamashita spectral types and corresponding effective temperature fit.\label{tab_YamashitaData}}

%% This command over-rides LaTeX's natural table count
%% and replaces it with this number.  LaTeX will increment
%% all other tables after this table based on this number


%% The \tablehead gives provides the column headers.  It
%% is currently set up so that the column labels are on the
%% top line and the units surrounded by ()s are in the
%% bottom line.  You may add more header information by writing
%% another line between these lines. For each column that requries
%% extra information be sure to include a \colhead{text} command
%% and remember to end any extra lines with \\ and include the
%% correct number of &s.
\tablehead{
Star ID & Yamashita & $T_{\rm EFF}$ & $T_{\rm EFF,fit}$ & $\Delta T$ \\
 & Sp Type\tablenotemark{a} & (K) & (K)\tablenotemark{b}  & (K)
}
%% All data must appear between the \startdata and \enddata commands
\startdata
HD225217 & C6,4 & $2989 \pm 102 $ & 2883 & 106 \\
HD2342 & C5,4 & $2808 \pm 95 $ & 2767 & 41 \\
HD19881 & C7,4 & $3314 \pm 113 $ & 3000 & 314 \\
IRC+40067 & C6,3 & $2606 \pm 89 $ & 2883 & -278 \\
HD30443 & C4,3 CH4: CN2: Ba4 & $3884 \pm 161 $ & 2680 & 1203 \\
HD280188 & C8,1J & $3361 \pm 114 $ & 3116 & 245 \\
HD33016 & C5,4 & $2727 \pm 93 $ & 2767 & -40 \\
HD34467 & C6,3 & $3003 \pm 102 $ & 2883 & 120 \\
HIP25004 & C4:,4 & $2715 \pm 92 $ & 2650 & 64 \\
HD38218 & C5,4 & $2710 \pm 92 $ & 2767 & -57 \\
HD247224 & C5,4 & $3056 \pm 104 $ & 2767 & 290 \\
HD38572 & C7,2 & $3483 \pm 118 $ & 3000 & 483 \\
HD38521 & C4,4 & $2580 \pm 88 $ & 2650 & -70 \\
HIP29896 & C5,4e: & $2597 \pm 88 $ & 2767 & -170 \\
HD45087 & C5,4 & $2723 \pm 92 $ & 2767 & -44 \\
HIP31349 & C8,3e & $3208 \pm 109 $ & 3116 & 91 \\
HD46321 & C4,5 & $2794 \pm 95 $ & 2650 & 143 \\
HD47883 & C5,4 Ba5 & $3118 \pm 106 $ & 2767 & 351 \\
HD48664 & C4,5 & $2612 \pm 89 $ & 2650 & -38 \\
HD51620 & C4,4 MS2 & $3290 \pm 112 $ & 2650 & 640 \\
HD54361 & C6,3 & $2907 \pm 99 $ & 2883 & 23 \\
IRC+10158 & C5,5 & $2561 \pm 87 $ & 2767 & -206 \\
HD57160 & C5,4J & $2871 \pm 98 $ & 2767 & 104 \\
HD59643 & C6,2 CH3 & $3775 \pm 128 $ & 2905 & 870 \\
HD60826 & C5,5 & $2694 \pm 92 $ & 2767 & -73 \\
HD70072 & C6,4e & $2381 \pm 81 $ & 2883 & -502 \\
HD144578 & C8,1e & $3450 \pm 117 $ & 3116 & 334 \\
HD173291 & C7,4 & $2793 \pm 95 $ & 3000 & -207 \\
HIP92194 & C5,4 & $2803 \pm 95 $ & 2767 & 36 \\
HIP95024 & C4,5e & $2483 \pm 84 $ & 2650 & -167 \\
HIP95777 & C4,5 & $2798 \pm 95 $ & 2650 & 148 \\
HD186047 & {\it C6.5,y} & $2878 \pm 98 $ & $-$ & $-$ \\
HIP99336 & C6,3e & $2924 \pm 113 $ & 2883 & 40 \\
HD191783 & C6,4 & $2796 \pm 95 $ & 2883 & -88 \\
HIP102764 & C6,4 & $2705 \pm 92 $ & 2883 & -178 \\
HIP105539 & C6,3e & $2703 \pm 92 $ & 2883 & -181 \\
IRC+50399 & {\it C7,y} & $3006 \pm 103 $ & $-$ & $-$ \\
HD208512 & C5,4e: & $2691 \pm 91 $ & 2767 & -75 \\
HD208526 & C4,4J MS5 & $2804 \pm 95 $ & 2650 & 154 \\
HIP113715 & C3,5J j6 MS6 & $2510 \pm 85 $ & 2534 & -24 \\
HD220870 & C7,3 & $2886 \pm 98 $ & 3000 & -114
\enddata
\tablenotetext{a}{Values in italics predicted from measured $T_{\rm EFF}$ and Equation \ref{eqn_YamTeffFit2} for those stars (HD186047, IRC+50399) for which no Yamashita spectra type was given.}
\tablenotetext{b}{From Equation \ref{eqn_YamTeffFit2}, which excludes CH carbon stars HD30443 and HD59643.}

%% Include any \tablenotetext{key}{text}, \tablerefs{ref list},
%% or \tablecomments{text} between the \enddata and
%% \end{deluxetable} commands

%% No \tablecomments indicated

%% No \tablerefs indicated

\end{deluxetable}
%\end{deluxetable*}
%\end{document}

